Identifying Spurious Biases Early in Training through the Lens of Simplicity Bias

Neural networks trained with (stochastic) gradient descent have an inductive bias towards learning simpler solutions. This makes them highly prone to learning spurious correlations in the training data, that may not hold at test time. In this work, we provide the first theoretical analysis of the effect of simplicity bias on learning spurious correlations. Notably, we show that examples with spurious features are provably separable based on the model's output early in training. We further illustrate that if spurious features have a small enough noise-to-signal ratio, the network's output on the majority of examples is almost exclusively determined by the spurious features, leading to poor worst-group test accuracy. Finally, we propose SPARE, which identifies spurious correlations early in training and utilizes importance sampling to alleviate their effect. Empirically, we demonstrate that SPARE outperforms state-of-the-art methods by up to 21.1% in worst-group accuracy, while being up to 12x faster. We also show that SPARE is a highly effective but lightweight method to discover spurious correlations.

==> defs.tex <==

\def\[#1\]{\begin{align}#1\end{align}}
\def\*[#1\]{\begin{align*}#1\end{align*}}


\newcommand{\loss}{\ell}
\newcommand{\weights}{w}
\newcommand{\wt}[1]{w_{#1}}
\newcommand{\wstacked}{\bm{w}}
\newcommand{\iid}{i.i.d.\xspace}

\newcommand{\Reals}{\mathbb{R}}

\newcommand{\Data}{\mathcal{D}}
\newcommand{\coreset}{\bar \Data}

\newcommand{\Jacob}[1]{\mathcal{J}(#1)}

\newcommand{\nnet}{\mathcal{N}}

\newcommand{\grad}{\nabla}

\newcommand{\dee}{\mathrm{d}}

\newcommand{\wdif}[1]{\Delta_{#1}}


\newcommand{\RiskChar}{\mathcal{L}}
\newcommand{\Risk}[2]{\RiskChar_{#1}\optparen{#2}}
\newcommand{\EmpRisk}[2]{\hat \RiskChar_{#1}\optparen{#2}}


\newcommand{\defn}[1]{\textit{#1}}

\newcommand{\warmup}{warm-up period\xspace}
\newcommand{\Warmup}{Warm-up period\xspace}
\newcommand{\interval}{interval\xspace}
\newcommand{\frequency}{frequency\xspace}
\newcommand{\rate}{sparsification level\xspace}
\newcommand{\rates}{sparsification levels\xspace}
\newcommand{\alg}{\textsc{GraTer}\xspace}
\newcommand{\algsgm}{\textsc{GraTer}\xspace}

\newcommand{\exemplars}{exemplars\xspace}
\newcommand{\onthefly}{on-the-fly\xspace}


\newcommand{\GTM}{\textsc{Gradient Trajectory Sparsification}\xspace}
\newcommand{\SGM}{\alg\xspace}



==> math_commands.tex <==

\usepackage{amsmath,amsfonts,bm}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/1_intro.tex <==
\vspace{-2mm}
\section{Introduction}
\vspace{-2mm}
The \textit{simplicity bias} of gradient-based training algorithms towards learning simpler solutions has been suggested as a key factor for the superior generalization performance of overparameterized neural networks \citep{hermann2020shapes,hu2020surprising,nakkiran2019sgd,neyshabur2014search,pezeshki2021gradient,shah2020pitfalls}.
At the same time, it is conjectured to make neural networks vulnerable to learning \textit{spurious correlations} frequently found in real-world datasets \citep{sagawa2019distributionally,sohoni2020no}. 
Neural networks trained with gradient-based methods can exclusively rely on
\textit{spurious features} that 
exist in more examples in one class than in other classes
but are not predictive of the class in general (e.g., image background for object classification),
and remain invariant to the predictive but more complex \textit{core features} 
\citep{shah2020pitfalls}. 
This results in learning non-robust solutions that do not generalize well 
on groups where the spurious correlations do not hold (e.g., the same object with an uncommon background)
\citep{shah2020pitfalls,teney2022evading}. \looseness=-1

Models can be trained to be robust against spurious correlations if \textbf{groups of examples without spurious correlation (NSG)} are upweighted \citep{sagawa2019distributionally} or upsampled \citep{liu2021just}  to counteract the influence of \textbf{groups with spurious correlation (SG)}. However, such robust training cannot be applied directly to real-world datasets because such grouping of data is usually unknown. To infer the groups, existing methods train a reference model via gradient descent and try to find NSG
based on misclassification \citep{liu2021just}, high loss \citep{nam2020learning,creager2021environment}, or sensitive representations \citep{sohoni2020no}. 
However, 
these methods are very sensitive to hyperparameters \cite{liu2021just,creager2021environment} and therefore heavily rely on extensive hyperparameter tuning with a group-labeled validation set for group inference.
Moreover, they are computationally expensive for either group inference \citep{sohoni2020no} or robust training \citep{taghanaki2021robust} or both \citep{liu2021just,nam2021spread,zhang2022correct} (as evidenced by \cref{tab:spurious}), rendering them impractical for even medium-sized datasets, not to mention when costs are further scaled by hyperparameter tuning. \yu{Most importantly, evidenced by our experiments, even with extensive hyperparameter tuning, these methods often fail to separate SG and NSG, whenever there is a significant class imbalance, or the spurious feature has a strong signal or a high noise.}
\looseness=-1

In this work, we show that, 
the simplicity bias of gradient descent, which leads to learning spurious 
correlations can be leveraged to provably separate SG and NSG
early in training to largely improve the group inference \yu{accuracy, and efficiency without} the need for extensive hyperparameter tuning.
We examine a two-layer fully connected neural network and identify two 
training phases in the presence of spurious features -- \textbf{scaling} and \textbf{domination}. 
\textit{Early in training,}
the spurious feature's contribution to the model's output within 
SG \textit{scales} linearly with the strength of the spurious correlation, making the model's output \textit{provably}  separates SG and NSG. Afterward, if the noise-to-signal ratio of a spurious feature is lower than that of the core feature, the model's output for most examples in the class becomes \textit{dominated}
by the spurious feature and therefore prevent the learning of the core feature. 
To the best of our knowledge, this is the first analysis of how the simplicity bias of SGD encourages learning of 
spurious correlations and inhibits learning of
core features. 

Based on these insights, we introduce an efficient yet effective method, \alg (\fullname), that clusters model output early in training to 
identify groups and further balance them with importance sampling to effectively improve the test accuracy of the robust model on NSG, without significantly sacrificing the average test accuracy on all examples or
increasing the training time. 
We first apply \alg to Restricted ImageNet, 
a dataset having no known spurious correlations and therefore no group-labeled validation set available for hyperparameter tuning,
to discover spurious correlations in more realistic settings beyond carefully curated benchmark datasets: \alg identifies up to 7.3\% more examples with spurious correlations than the state-of-the-art group inference methods and improves model's accuracy on NSG by
up to 23.2\% higher than them after robust training.
Then, %
we confirm that \alg can achieve up to 5.6\% higher worst-group accuracy compared to state-of-the-art baselines on multiple most commonly used benchmark datasets, including CMNIST \citep{alain2015variance}, Waterbirds \citep{sagawa2019distributionally}, and CelebA \citep{liu2015faceattributes} while being up to 12x faster. 
 \looseness=-1


==> sections/2_related.tex <==
\vspace{-2mm}
\section{Related Work}\label{sec:related}
\vspace{-2mm}
\textbf{Identifying and mitigating spurious correlations.}
If group labels are available at training time, techniques such as class balancing \citep{he2009learning,cui2019class} and importance weighting \citep{shimodaira2000improving,byrd2019effect} 
are used to enhance performance on minority groups. Alternatively, GDRO \citep{sagawa2019distributionally} focuses on higher-loss groups to minimize the worst group-level error.
Without group labels, existing methods aim to first \yu{train an inference model to} infer this information for \yu{the robust}
model training. GEORGE \citep{sohoni2020no} \yu{clusters feature representations of a model fully trained with} ERM  (Empirical Risk Minimization) and then trains the \yu{robust} model with GDRO. 
LfF \citep{nam2020learning} trains two models simultaneously; the second model upweights examples with high loss from the first. 
JTT \citep{liu2021just} \yu{similarly trains an ERM model but for fewer epochs, then}
upsample examples
misclassified by this reference model and trains the robust model using ERM \yu{with the upsampled training set}.
EIIL \citep{creager2021environment} and PGI \citep{ahmed2020systematic} also split data based on a reference ERM model but by finding an assignment that maximizes the Invariant Risk Minimization (IRM) objective \citep{arjovsky2017towards}, i.e., the variance of the model on the two groups. Then, EIIL trains the robust model with GDRO, and PGI minimizes the KL divergence of softmaxed logits for same-class samples across groups. 
\looseness=-1

These state-of-the-art methods heavily rely on extra group-labeled data \citep{nam2021spread,kirichenko2023last} to tune their %
group inference method in a wider range of hyperparameters, 
\yu{and often fail to find spurious features when the classes are highly imbalanced, or when the signal or the noise of the spurious feature is too large.}
Besides, they often significantly increase training time during group-inference or robust training \citep{liu2021just,nam2021spread,zhang2022correct}. In contrast, \alg can \textit{provably} and accurately separate groups of examples with spurious features \textit{early} in training, thus does not require extensive hyperparameter tuning, and yields a superior performance on minority groups without increasing the training time.
\looseness=-1



\textbf{Simplicity 
Bias.}
Recent work has revealed the simplicity bias in (stochastic) gradient methods towards learning linear functions early in training, progressing to more complex functions later \citep{hermann2020shapes,hu2020surprising,nakkiran2019sgd,neyshabur2014search,pezeshki2021gradient,shah2020pitfalls}. This is empirically observed in various network architectures, including MobileNetV2, ResNet50, and DenseNet121 \citep{sandler2018mobilenetv2,he2016deep,shah2020pitfalls}. \cite{hu2020surprising} formally proved that initial learning dynamics of a two-layer FC network can be mimicked by a linear model and extended this to multi-layer FC and convolutional networks. Simplicity bias is suggested to explain the good generalization of overparameterized networks but is also \textit{conjectured} to produce models that rely on the simplest feature at the expense of more complex ones, even when the simplest feature has less predictive power \citep{shah2020pitfalls,teney2022evading}. However, the exact notion of the simplicity of features and the mechanism by which they are learned remain poorly understood except in certain simplistic settings \citep{nagarajan2020understanding,shah2020pitfalls}. Here, we build on \cite{hu2020surprising} and rigorously specify the required conditions and mechanism of learning spurious features by a two-layer FC network.





